Helium Variation Across Two Solar Cycles Reveals A Speed-Dependent Phase Lag

We study the relationship between solar wind helium to hydrogen abundance ratio ($A_\mathrm{He}$), solar wind speed ($v_\mathrm{SW}$), and sunspot number (SSN) over solar cycles 23 and 24. This is the first full 22-year Hale cycle measured with the Wind spacecraft covering a full cycle of the solar dynamo with two polarity reversals. While previous studies have established a strong correlation between $A_\mathrm{He}$ and SSN, we show that the phase delay between $A_\mathrm{He}$ and SSN is a monotonic increasing function of $v_\mathrm{SW}$. Correcting for this lag, $A_\mathrm{He}$ returns to the same value at a given SSN over all rising and falling phases and across solar wind speeds. We infer that this speed-dependent lag is a consequence of the mechanism that depletes slow wind $A_\mathrm{He}$ from its fast wind value during solar wind formation.

==> preamble/journal_specific.tex <==
%=============================
%Dates, submitted journal, etc
%=============================
%% Reintroduced the \received and \accepted commands from AASTeX v5.2
\received{January 1, 2018}
\revised{January 7, 2018}
\accepted{\today}
%% Command to document which AAS Journal the manuscript was submitted to.
%% Adds "Submitted to " the arguement.
\submitjournal{ApJL}

==> sections/stale/discussion.tex <==
\section{Discussion}\label{sec:disc}
\input{sections/he-filtration}
\input{sections/xcorr-sig}

==> sections/stale/scratch.tex <==
\section{Scratch Notes} \label{sec:scratch}

\subsection{From \sect{intro}}

While the specific physical mechanism driving \ahe's variation with \vsw\ and \ssn\ is unknown,  it has been interpreted as a signature of variation in the sources of the solar wind in the ecliptic plane and changes in the coronal plasma above those source regions.
\question{For example, minor ion charge state reflect the corona's temperature, \citep{????} which varies as a function with solar cycle \citep{????}.}
\citet{Kasper2012} \question{showed something about how minor ion charge state indicates XXXX about \ahe}.
Additionally, \ahe\ is known to vary with heliographic latitude, which may indicate source-surface variation drives alpha-proton differential flow. \citep{Kasper2007}
\citet{McIntosh2011a} demonstrated that the variation in \ahe\ detected by \citet{Kasper2007} may be related to variation in scale size in the solar transition region.
\question{\citet{????} showed that the variation of \vsw\ with solar cycle is at least partially driven by XXXXX.}
\ben{The previous sentence should tie us back it \xcorr.}
\dnc{Now, with multiple solar cycles, we are able to detect a speed dependent lag between a change \ssn\ and solar wind \ahe.}


\question{Something about the variation of heavier ions being tied to changes in the corona.
One sentence on charge states.
One sentence on FIP and/or freeze-in temperatures.}

Excluding transient events (e.g. coronal mass ejections (CMEs) and stream interaction), the source of \ahe variation is unknown, especially at long timescale.

To low order, there are two classes of solar wind: slow and fast.
Fast solar wind ($\vsw \gtrsim 500 \; \kms$) originates from (polar) coronal holes. \citep{????}
\question{It has several known properties.}
Slow wind typically to refer to solar wind with $\vsw \lesssim 500 \; \kms$) and typically refers to solar wind that is equatorial in origin, especially from active regions, helmet streamers, and the heliospheric current sheet. \cite{????,????}
Some authors further divide the solar wind into three classes: slow ($\vsw \lesssim 400 \; \kms$), intermediate ($400 \; \kms \lesssim \vsw \lesssim 600 \; \kms$), and fast ($\vsw \gtrsim 600 \; \kms$).
While the differentiation of solar wind type by \vsw\ is typically considered an over simplification that neglects more fundamental physics at the solar wind's origin, \citep{Something about the S-Web? Something about various charge states? Something about fractionation?} to low-order \vsw\ does correlate with these various mechanisms.
For example, \citet{Kasper2012} showed that \ahe\ varies with minor ion charge state.
Additionally, alpha and proton measurements are made concurrently on \Wind.
As such, using it as a classification scheme reduces systematic uncertainties and provides a more reliable and simpler to access tool than any other mechanism.

The \Wind\ spacecraft launched in 1994.
Since that time, the Solar Wind Experiment (SWE) Faraday cups (FC)


In this Letter, we examine the long term variation of \ahe\ with \vsw\ and \ssn.


This Letter investigates the variation of \xcorr\ with \vsw\


Many arguments have been made regarding the variation of \ahe\ with solar cycle.
The most prominent and believable center on the variation being tied to variations at the solar source.


\question{The supergranular network is XXXXXX.
It correlates/constitutes some measurement of the transition region.}
\citet{McIntosh2011c} measured this network's scale size and \citet{McIntosh2011a} have shown that the variation of \ahe\ with \vsw\ and \ssn\ found in \citet{Kasper2007,Kasper2012} co-varies with this scale size.



\citet{Ogilvie1974} suggest a relationship between \ahe\ and \vsw.

\question{Something, something, something... delay in change of helium due to something solar surface  something diffusion.}

For simplicity, we label the cross correlation coefficient between \ahe\ and \ssn\ with \xcorr.

Something about \citet{Kasper2007} latitudinal variation.
Something about \citet{McIntosh2011a} publishing a comparison to transition region (i.e.\ supergranular) network length scale.
Something about \citet{Kasper2012} minor ion evolution.
